Query-Conditioned Graph Retrieval for Contextualized LLM Reasoning in Personalized Wearable Data

Large language models (LLMs) are increasingly applied to analyzing wearable sensing data, which are long-term, multimodal, and highly personalized. A key challenge is context selection: providing insufficient context limits reasoning, while including all available data leads to inefficiency and degraded generation quality. We propose Wearable As Graph (WAG), a graph-based context retrieval framework that enables query-adaptive reasoning over wearable data with LLMs. WAG organizes wearable metrics and user-specific signals into a personalized knowledge graph, and retrieves a query-conditioned subgraph to support downstream generation. The retrieval process integrates global relationships, capturing prior knowledge and population- and individual-level patterns via hierarchical Bayesian modeling, with local relationships that reflect short-term signal deviations. A query openness signal further controls retrieval breadth. We evaluate WAG on over 10,000 data-grounded queries from real-world wearable datasets. Across LLM-based and human evaluations, WAG achieves an approximately 70% win rate over baseline and standard RAG methods, demonstrating the effectiveness of structured, query-adaptive context retrieval for LLM-driven analysis of wearable data.

==> app/detailed_method2.tex <==
\section{Detailed Method}
\subssection{Detailed derivation: Hierarchical Bayesian update with Fisher \(z\)-transform}

\subsection{Notation and Fisher \(z\)-transform}
Let \(x\) be a primary node and \(Y=\{y_1,\dots,y_{|Y|}\}\) its neighbors.
We model the subject-specific relationship-strength vector
\(\boldsymbol{\theta}_x^i = [\theta_{x,y_1}^i,\dots,\theta_{x,y_{|Y|}}^i]^\top\).
Observed correlation summaries are
\(\boldsymbol{R}_x^{\mathrm{pop}} = [r_{x,y_1}^{\mathrm{pop}},\dots,r_{x,y_{|Y|}}^{\mathrm{pop}}]^\top\)
and
\(\boldsymbol{R}_x^{i} = [r_{x,y_1}^{i},\dots,r_{x,y_{|Y|}}^{i}]^\top\).

We apply the Fisher \(z\)-transform elementwise:
\[
\boldsymbol{Z}_x^{\mathrm{pop}} = \operatorname{arctanh}(\boldsymbol{R}_x^{\mathrm{pop}}), \qquad
\boldsymbol{Z}_x^{i} = \operatorname{arctanh}(\boldsymbol{R}_x^{i}),
\]
where for a scalar \(r\),
\[
z=\operatorname{arctanh}(r)=\tfrac12\ln\!\left(\frac{1+r}{1-r}\right),\qquad r=\tanh(z).
\]
On the \(z\)-scale an individual transformed correlation \(z\) is approximately
\(\mathcal{N}(\operatorname{arctanh}(\rho),\; 1/(n-3))\) for Pearson; for Spearman use the appropriate variance adjustment.  
We will denote the sampling-covariance matrices on the \(z\)-scale by \(\boldsymbol{V}_x^{\mathrm{pop}}\) and \(\boldsymbol{V}_x^{i}\) (commonly diagonal with \([\,\boldsymbol{V}]_{jj}\approx 1/(n_j-3)\)).

\subsection*{Model (on the Fisher-\(z\) scale)}
We place a Gaussian prior on the latent \(z\)-parameters (i.e., on \(\boldsymbol{\theta}_x^i\) interpreted on the \(z\)-scale):
\[
\boldsymbol{\theta}_x^i \sim \mathcal{N}(\boldsymbol{\mu}_x^{\mathrm{prior}},\, \boldsymbol{\Sigma}_x^{\mathrm{prior}}).
\]
Population and individual observed \(z\)-vectors are modeled as noisy observations of \(\boldsymbol{\theta}_x^i\):
\[
\boldsymbol{Z}_x^{\mathrm{pop}} \mid \boldsymbol{\theta}_x^i \sim \mathcal{N}(\boldsymbol{\theta}_x^i,\; \boldsymbol{V}_x^{\mathrm{pop}}),\qquad
\boldsymbol{Z}_x^{i} \mid \boldsymbol{\theta}_x^i \sim \mathcal{N}(\boldsymbol{\theta}_x^i,\; \boldsymbol{V}_x^{i}).
\]
Assume conditional independence:
\(\boldsymbol{Z}_x^{\mathrm{pop}} \perp \boldsymbol{Z}_x^{i} \mid \boldsymbol{\theta}_x^i\).

\subsection*{Bayes' rule (combined posterior)}
From Bayes' theorem:
\[
p(\boldsymbol{\theta}_x^i \mid \boldsymbol{Z}_x^{\mathrm{pop}},\boldsymbol{Z}_x^{i})
\propto p(\boldsymbol{Z}_x^{\mathrm{pop}}\mid\boldsymbol{\theta}_x^i)\,
p(\boldsymbol{Z}_x^{i}\mid\boldsymbol{\theta}_x^i)\, p(\boldsymbol{\theta}_x^i).
\]
Plugging in the Gaussian densities (writing only the exponential-quadratic terms):
\begin{align*}
p(\boldsymbol{\theta}_x^i \mid \cdots)
&\propto
\exp\Big(-\tfrac{1}{2}(\boldsymbol{Z}_x^{\mathrm{pop}}-\boldsymbol{\theta}_x^i)^\top (\boldsymbol{V}_x^{\mathrm{pop}})^{-1}(\boldsymbol{Z}_x^{\mathrm{pop}}-\boldsymbol{\theta}_x^i)\Big) \\
&\quad\times
\exp\Big(-\tfrac{1}{2}(\boldsymbol{Z}_x^{i}-\boldsymbol{\theta}_x^i)^\top (\boldsymbol{V}_x^{i})^{-1}(\boldsymbol{Z}_x^{i}-\boldsymbol{\theta}_x^i)\Big) \\
&\quad\times
\exp\Big(-\tfrac{1}{2}(\boldsymbol{\theta}_x^i-\boldsymbol{\mu}_x^{\mathrm{prior}})^\top (\boldsymbol{\Sigma}_x^{\mathrm{prior}})^{-1}(\boldsymbol{\theta}_x^i-\boldsymbol{\mu}_x^{\mathrm{prior}})\Big).
\end{align*}

\subsection*{Complete-the-square: posterior is Gaussian}
Collect the quadratic and linear terms in \(\boldsymbol{\theta}_x^i\).
Define precisions (inverse covariances):
\[
\boldsymbol{\Lambda}^{\mathrm{prior}}=(\boldsymbol{\Sigma}_x^{\mathrm{prior}})^{-1},\quad
\boldsymbol{\Lambda}^{\mathrm{pop}}=(\boldsymbol{V}_x^{\mathrm{pop}})^{-1},\quad
\boldsymbol{\Lambda}^{i}=(\boldsymbol{V}_x^{i})^{-1}.
\]
The quadratic form in the exponent becomes
\[
-\tfrac12\,(\boldsymbol{\theta}_x^i)^\top\!\big(\boldsymbol{\Lambda}^{\mathrm{prior}}+\boldsymbol{\Lambda}^{\mathrm{pop}}+\boldsymbol{\Lambda}^{i}\big)\boldsymbol{\theta}_x^i
+\big(\boldsymbol{\Lambda}^{\mathrm{prior}}\boldsymbol{\mu}_x^{\mathrm{prior}}
+\boldsymbol{\Lambda}^{\mathrm{pop}}\boldsymbol{Z}_x^{\mathrm{pop}}
+\boldsymbol{\Lambda}^{i}\boldsymbol{Z}_x^{i}\big)^\top\!\boldsymbol{\theta}_x^i
+\text{(terms not depending on }\boldsymbol{\theta}_x^i).
\]
Thus the posterior is multivariate normal with precision matrix
\[
\boldsymbol{\Lambda}^{\mathrm{post}}=\boldsymbol{\Lambda}^{\mathrm{prior}}+\boldsymbol{\Lambda}^{\mathrm{pop}}+\boldsymbol{\Lambda}^{i},
\]
and covariance
\[
\boxed{\qquad
\boldsymbol{\Sigma}_x^{i} \;=\; (\boldsymbol{\Lambda}^{\mathrm{post}})^{-1}
\;=\; \Big((\boldsymbol{\Sigma}_x^{\mathrm{prior}})^{-1} + (\boldsymbol{V}_x^{\mathrm{pop}})^{-1} + (\boldsymbol{V}_x^{i})^{-1}\Big)^{-1}. \qquad}
\]
The posterior mean is the precision-weighted sum:
\[
\boxed{\qquad
\boldsymbol{\mu}_x^{i} \;=\; \boldsymbol{\Sigma}_x^{i}\big(
(\boldsymbol{\Sigma}_x^{\mathrm{prior}})^{-1}\boldsymbol{\mu}_x^{\mathrm{prior}}
+ (\boldsymbol{V}_x^{\mathrm{pop}})^{-1}\boldsymbol{Z}_x^{\mathrm{pop}}
+ (\boldsymbol{V}_x^{i})^{-1}\boldsymbol{Z}_x^{i}
\big). \qquad}
\]

\paragraph{Sequential (two-stage) derivation.}
It is often convenient to perform the updates sequentially.

\textbf{Stage 1 (population)}:
\[
\boldsymbol{\Sigma}_x^{\mathrm{pop}}=\Big((\boldsymbol{\Sigma}_x^{\mathrm{prior}})^{-1}+(\boldsymbol{V}_x^{\mathrm{pop}})^{-1}\Big)^{-1},\qquad
\boldsymbol{\mu}_x^{\mathrm{pop}}=\boldsymbol{\Sigma}_x^{\mathrm{pop}}\Big(
(\boldsymbol{\Sigma}_x^{\mathrm{prior}})^{-1}\boldsymbol{\mu}_x^{\mathrm{prior}}
+(\boldsymbol{V}_x^{\mathrm{pop}})^{-1}\boldsymbol{Z}_x^{\mathrm{pop}}
\Big).
\]

\textbf{Stage 2 (subject)}: treat \( \mathcal{N}(\boldsymbol{\mu}_x^{\mathrm{pop}},\boldsymbol{\Sigma}_x^{\mathrm{pop}}) \) as the prior and update with \(\boldsymbol{Z}_x^{i}\):
\[
\boldsymbol{\Sigma}_x^{i}=\Big( (\boldsymbol{\Sigma}_x^{\mathrm{pop}})^{-1}+(\boldsymbol{V}_x^{i})^{-1}\Big)^{-1},\qquad
\boldsymbol{\mu}_x^{i}=\boldsymbol{\Sigma}_x^{i}\Big(
(\boldsymbol{\Sigma}_x^{\mathrm{pop}})^{-1}\boldsymbol{\mu}_x^{\mathrm{pop}}
+(\boldsymbol{V}_x^{i})^{-1}\boldsymbol{Z}_x^{i}
\Big).
\]
Substituting \((\boldsymbol{\Sigma}_x^{\mathrm{pop}})^{-1}=(\boldsymbol{\Sigma}_x^{\mathrm{prior}})^{-1}+(\boldsymbol{V}_x^{\mathrm{pop}})^{-1}\)
recovers the single-step formulas above, showing algebraic equivalence.

\subsection*{Transforming the posterior back to correlation space}
The posterior \(\mathcal{N}(\boldsymbol{\mu}_x^{i},\boldsymbol{\Sigma}_x^{i})\) is on the Fisher-\(z\) scale.
To obtain point estimates of correlations, apply the elementwise inverse transform:
\[
\widehat{\boldsymbol{R}}_x^i \;=\; \tanh(\boldsymbol{\mu}_x^{i})
\qquad\text{(elementwise)}.
\]
If an approximate posterior variance on the correlation scale is desired, use the delta method:
for the \(j\)-th element with posterior mean \(\mu_{j}\) and variance \(\sigma_{j}^2\) on the \(z\)-scale,
\[
\operatorname{Var}[\tanh(z)] \approx \big(\operatorname{sech}^2(\mu_{j})\big)^2 \sigma_{j}^2
= \big(1-\tanh^2(\mu_{j})\big)^2 \sigma_{j}^2,
\]
where \(\operatorname{sech}(u)=1/\cosh(u)\).

% \subsection*{Implementation notes and assumptions}
% \begin{itemize}
%   \item \textbf{Diagonal vs full covariance:} The derivation above is valid in the multivariate case for arbitrary positive-definite \(\boldsymbol{V}\) and \(\boldsymbol{\Sigma}\). In practice, one often assumes \(\boldsymbol{V}_x^{\mathrm{pop}}\) and \(\boldsymbol{V}_x^{i}\) are diagonal (independent \(z\)-estimates across edges) with diagonal entries \(\approx 1/(n_j-3)\). If edges are correlated, supply full covariance estimates and the formulas remain unchanged.
%   \item \textbf{Spearman correlations:} For Spearman correlations the Fisher-\(z\) approximation and variance \(1/(n-3)\) are only approximate; apply empirical variance adjustments or bootstrap-based variances for improved accuracy.
%   \item \textbf{Numerical stability:} work in precision form when possible (add precisions), and regularize covariances to ensure positive-definiteness (e.g., add small diagonal ridge).
% \end{itemize}

% \qed
% Our method is not a typical \textbf{fully generative hierarchical Bayesian model}. In a standard formulation, the \textit{population distribution} \$(\textbackslash{}mu\_x, \textbackslash{}Sigma\_x)\$ is treated as a set of latent hyperparameters with their own priors, and inference is carried out via MCMC or variational methods. While this approach is flexible, it typically requires computationally intensive sampling, which must be repeated at inference time. We believe such sampling is not appropriate for our setting, where repeated, efficient inference is required.

% Instead, our approach adopts a \textbf{simplified empirical Bayes formulation} with closed-form Gaussian updates. This allows us to retain the population-to-individual hierarchy while ensuring computational tractability.

\subsection{Global Modeling-HBM derivation}
\section{Hierarchical Bayesian Modeling (HBM)}
\label{sec:hbm}
This provides a comprehensive derivation of the posterior distribution for the latent long-term edge weight vector $\Theta_x^s$ for a subject $s$ and source node $x$. The model integrates a prior distribution, population-level data, and individual-level data within a conjugate Gaussian framework.
\[
\Theta_x^s = [\theta_{x,y_1}^s,\dots,\theta_{x,y_{|Y|}}^s]^\top \in \mathbb{R}^{|Y|}
\]


\subsection*{Model specification}
\begin{align}
\Theta_x^s &\sim \mathcal{N}(\mu_x^{\text{prior}}, \Sigma_x^{\text{prior}}), \\
R_x^{\text{pop}} \mid \Theta_x^s &\sim \mathcal{N}(\Theta_x^s, V_x^{\text{pop}}), \\
R_x^{s} \mid \Theta_x^s &\sim \mathcal{N}(\Theta_x^s, V_x^{s}),
\end{align}
where $R_x^{\text{pop}},R_x^s,\mu_x^{\text{prior}}\in\mathbb{R}^{|Y|}$ and $\Sigma_x^{\text{prior}},V_x^{\text{pop}},V_x^s$ are covariance matrices.

By Bayes' rule and conditional independence of the two observation sources given \(\Theta_x^s\),
\[
p(\Theta_x^s\mid R_x^{\mathrm{pop}},R_x^s) \propto p(\Theta_x^s)\,p(R_x^{\mathrm{pop}}\mid\Theta_x^s)\,p(R_x^s\mid\Theta_x^s).
\]
The (negative) log of the  posterior as follows:
\[
\begin{aligned}
\mathcal{L}(\Theta) &\equiv -\log p(\Theta_x^s\mid R_x^{\mathrm{pop}},R_x^s) + C \\
&= \tfrac{1}{2}(\Theta-\mu^{\mathrm{prior}})^\top (\Sigma^{\mathrm{prior}})^{-1}(\Theta-\mu^{\mathrm{prior}}) \\
&\quad + \tfrac{1}{2}(R^{\mathrm{pop}}-\Theta)^\top (V^{\mathrm{pop}})^{-1}(R^{\mathrm{pop}}-\Theta) \\
&\quad + \tfrac{1}{2}(R^{s}-\Theta)^\top (V^{s})^{-1}(R^{s}-\Theta),
\end{aligned}
\]
To simplify notation for the derivation, subscript \(x\) and superscript \(s\) inside this derivation are dropped: \(\Theta\equiv\Theta_x^s,\ \mu^{\mathrm{prior}}\equiv\mu_x^{\mathrm{prior}},\ R^{\mathrm{pop}}\equiv R_x^{\mathrm{pop}},\ R^s\equiv R_x^s,\) etc.


Expand each quadratic term and collect terms in \(\Theta\):
\[
\begin{aligned}
\mathcal{L}(\Theta)
&= \tfrac{1}{2}\Theta^\top (\Sigma^{\mathrm{prior}})^{-1}\Theta - (\Sigma^{\mathrm{prior}})^{-1}\mu^{\mathrm{prior}}\!^\top\Theta + \tfrac{1}{2}{\mu^{\mathrm{prior}}}^\top(\Sigma^{\mathrm{prior}})^{-1}\mu^{\mathrm{prior}} \\
&\quad + \tfrac{1}{2}\Theta^\top (V^{\mathrm{pop}})^{-1}\Theta - (V^{\mathrm{pop}})^{-1}R^{\mathrm{pop}}\!^\top\Theta + \tfrac{1}{2}{R^{\mathrm{pop}}}^\top (V^{\mathrm{pop}})^{-1} R^{\mathrm{pop}} \\
&\quad + \tfrac{1}{2}\Theta^\top (V^{s})^{-1}\Theta - (V^{s})^{-1}R^{s}\!^\top\Theta + \tfrac{1}{2}{R^{s}}^\top (V^{s})^{-1} R^{s}.
\end{aligned}
\]
Collecting the quadratic (in \(\Theta\)) and linear terms yields
\[
\mathcal{L}(\Theta) = \tfrac{1}{2}\Theta^\top \Lambda \,\Theta - b^\top \Theta + \text{const},
\]
where
\begin{align}
\Lambda &\equiv (\Sigma^{\mathrm{prior}})^{-1} + (V^{\mathrm{pop}})^{-1} + (V^{s})^{-1}, \label{eq:Lambda_def}\\
b &\equiv (\Sigma^{\mathrm{prior}})^{-1}\mu^{\mathrm{prior}} + (V^{\mathrm{pop}})^{-1}R^{\mathrm{pop}} + (V^{s})^{-1}R^{s}. \label{eq:b_def}
\end{align}

Complete the square for the quadratic form:
\[
\begin{aligned}
\mathcal{L}(\Theta)
&= \tfrac{1}{2}(\Theta^\top \Lambda \Theta - 2 b^\top \Theta) + \text{const} \\
&= \tfrac{1}{2}(\Theta - \Lambda^{-1} b)^\top \Lambda (\Theta - \Lambda^{-1} b) - \tfrac{1}{2} b^\top \Lambda^{-1} b + \text{const}.
\end{aligned}
\]
Therefore the posterior is Gaussian,
\[
\Theta_x^s \mid R_x^{\mathrm{pop}},R_x^s \sim \mathcal{N}(\mu,\Sigma),
\]
with
\begin{align}
\Sigma &= \Lambda^{-1} = \Big((\Sigma^{\mathrm{prior}})^{-1} + (V^{\mathrm{pop}})^{-1} + (V^{s})^{-1}\Big)^{-1}, \label{eq:Sigma_final}\\
\mu &= \Sigma\, b = \Sigma\Big((\Sigma^{\mathrm{prior}})^{-1}\mu^{\mathrm{prior}} + (V^{\mathrm{pop}})^{-1}R^{\mathrm{pop}} + (V^{s})^{-1}R^{s}\Big). \label{eq:mu_final}
\end{align}


\subsection{Local Modeling}





==> app/prompt_2.tex <==
\clearpage

% 关键修复：强制切换为单栏（跨栏），避免宽度错误
\onecolumn
\lstset{
    language=JSON,
    basicstyle=\scriptsize\ttfamily,  % 更小字体，适配跨栏宽度
    breaklines=true,                    % 强制换行，核心！
    frame=single,                       % 边框包裹
    captionpos=b,
    caption={Complete Prompt for Wearable Health Metric Question Generation},
    label={lst:health_prompt_cross},
    commentstyle=\color{gray},
    keywordstyle=\color{blue},
    numbers=left,
    numberstyle=\tiny\color{gray},
    columns=fullflexible,               % 自适应宽度
    keepspaces=true,                    % 保留空格/换行，防止内容压缩
    lineskip=-0.5pt,                    % 减小行距，完整显示内容
    xleftmargin=1em,                    % 左侧边距，避免内容贴边
    xrightmargin=1em                    % 右侧边距
}

\begin{lstlisting}
Generate diverse, clinically relevant questions about health metrics from wearable data.

INPUT FORMAT (Array of metric objects):
[
    {
        "id": "<unique_id>",
        "name": "<metric_name>",        # The health metric being analyzed
        "description": "<definition>",  # Clinical definition of the metric
        "date": "<YYYY-MM-DD>",
        "time_granularity": "<1|7|14|30|60|all>",  # Time period covered
        "abnormality_level": "<low|medium|high>", # Deviation from user's baseline
    },
    ...
]

OUTPUT FORMAT (Array of questions - one per input metric):
[
    {
        "id": "<matching_input_id>",
        "question": "<clear, time-bound phrasing>",
        "question_type": "<one of: General Knowledge | Data Retrieval | Trend Analysis | Comparative Insight | Anomaly Detection | Actionable Advice | Exploratory Analysis>",
        "openness": <0.0-1.0>,     # 0.0=closed, 1.0=open-ended
    },
    ...
]

QUESTION FRAMEWORK:
1. General Knowledge (Openness: 0.2-0.4)
   - Definitions, benchmarks, normal ranges
   - Example: "What's considered a healthy range for [metric]?" "What is [metric]?"

2. Data Retrieval (Openness: 0.1-0.3)
   - Specific time-bound numerical queries
   - Example: "What was my [metric] yesterday?" "What was my max/min/average [metric] this week?"

3. Trend Analysis (Openness: 0.4-0.6)
   - Patterns over days/weeks/months
   - Example: "Identify any trends in my [metric] over the last 30 days." "Summarize my [metric] for the past month."

4. Comparative Insight (Openness: 0.5-0.7)
   - Time-period comparisons
   - Example: "How does this week's [metric] compare to last week?"

5. Anomaly Detection (Openness: 0.6-0.8)
   - Statistical outliers
   - Example: "Were there unusual [metric] spikes in this month?"

6. Actionable Advice (Openness: 0.3-0.5)
   - Data-driven recommendations
   - Example: "What adjustments could improve my [metric]?"

7. Exploratory Analysis (Openness: 0.7-1.0)
   - Multi-factor investigations
   - Example: "Do you think I am stressed recently?" "I'm feeling really tired today. do you know why?" "Why might I be feeling tired despite sleeping 8 hours?"

GENERATION RULES:
1. Time binding:
   - Map granularity to natural terms:
     • 1 → "today"
     • 7 → "past 7 days"
     • 14 → "past 14 days"
     • 30 → "past 30 days"
     • 60 → "past 60 days"
     • all → "overall"
2. Blend concrete and exploratory questions per category:
   - 40% objective (openness ≤0.4)
   - 30% moderate (0.4 < openness <0.7)
   - 30% open-ended (≥0.7)
3. Prevent overlap between categories
4. For medium/high abnormalities, prioritize generating high openness questions
5. Exactly 1 output question per input group

EXAMPLES:
INPUT:
[
    {
        "id": "m001",
        "name": "Inactive time",  
        "description": "The amount of time a user is inactive, measured in minutes",
        "date": "2020-01-01",
        "time_granularity": "1",
        "abnormality_level": "low", 
    },
    {
        "id": "m002",
        "name": "total sleep time",  
        "description": "The total amount of time a user spends in sleep",
        "date": "2020-02-02",
        "time_granularity": "14",
        "abnormality_level": "high", 
    }
]

OUTPUT:
[
    {
        "id": "m001",
        "question": "What was my inactive time today?",
        "question_type": "Data Retrieval",
        "openness": 0.1,
    },
    {
        "id": "m002",
        "question": "How does my total sleep time over the past 14 days compare to the previous period?",
        "question_type": "Comparative Insight",
        "openness": 0.7,
    }
]
\end{lstlisting}

% 切回双栏，不影响后续附录内容
\twocolumn

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

